Learning Distributions on Manifolds with Free-Form Flows

We propose Manifold Free-Form Flows (M-FFF), a simple new generative model for data on manifolds. The existing approaches to learning a distribution on arbitrary manifolds are expensive at inference time, since sampling requires solving a differential equation. Our method overcomes this limitation by sampling in a single function evaluation. The key innovation is to optimize a neural network via maximum likelihood on the manifold, possible by adapting the free-form flow framework to Riemannian manifolds. M-FFF is straightforwardly adapted to any manifold with a known projection. It consistently matches or outperforms previous single-step methods specialized to specific manifolds. It is typically two orders of magnitude faster than multi-step methods based on diffusion or flow matching, achieving better likelihoods in several experiments. We provide our code at https://github.com/vislearn/FFF.

==> preamble.tex <==
\usepackage{amsthm}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\usepackage{lipsum}  

\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}

\usepackage{pifont}
\definecolor{myred}{RGB}{215,48,39}
\definecolor{mygreen}{RGB}{26,152,80}
\newcommand{\cmark}{\textcolor{mygreen}{\ding{51}}}
\newcommand{\xmark}{\textcolor{myred}{\ding{55}}}

\newcommand{\tr}{\operatorname{tr}}
\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\KL}{\operatorname{KL}}
\newcommand{\Diag}{\operatorname{Diag}}
\newcommand{\detM}{\det{}\!_\M}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\proj}{\operatorname{proj}}
\newcommand{\emb}{\operatorname{emb}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\M}{\Mm}
\newcommand{\T}{\Tt}
\renewcommand{\S}{\mathbb{S}}
\newcommand{\N}{\Nn}
\newcommand{\R}{\RR}
\newcommand{\E}{\EE}

\newcommand{\NN}{\mathbb{N}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}

\newcommand{\Aa}{\mathcal{A}}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dd}{\mathcal{D}}
\newcommand{\Ee}{\mathcal{E}}
\newcommand{\Ff}{\mathcal{F}}
\newcommand{\Gg}{\mathcal{G}}
\newcommand{\Hh}{\mathcal{H}}
\newcommand{\Ii}{\mathcal{I}}
\newcommand{\Jj}{\mathcal{J}}
\newcommand{\Kk}{\mathcal{K}}
\newcommand{\Ll}{\mathcal{L}}
\newcommand{\Mm}{\mathcal{M}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Oo}{\mathcal{O}}
\newcommand{\Pp}{\mathcal{P}}
\newcommand{\Qq}{\mathcal{Q}}
\newcommand{\Rr}{\mathcal{R}}
\newcommand{\Ss}{\mathcal{S}}
\newcommand{\Tt}{\mathcal{T}}
\newcommand{\Uu}{\mathcal{U}}
\newcommand{\Vv}{\mathcal{V}}
\newcommand{\Ww}{\mathcal{W}}
\newcommand{\Xx}{\mathcal{X}}
\newcommand{\Yy}{\mathcal{Y}}
\newcommand{\Zz}{\mathcal{Z}}

\newcommand{\aA}{\mathfrak{A}}
\newcommand{\bB}{\mathfrak{B}}
\newcommand{\cC}{\mathfrak{C}}
\newcommand{\dD}{\mathfrak{D}}
\newcommand{\eE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}
\newcommand{\gG}{\mathfrak{G}}
\newcommand{\hH}{\mathfrak{H}}
\newcommand{\iI}{\mathfrak{I}}
\newcommand{\jJ}{\mathfrak{J}}
\newcommand{\kK}{\mathfrak{K}}
\newcommand{\lL}{\mathfrak{L}}
\newcommand{\mM}{\mathfrak{M}}
\newcommand{\nN}{\mathfrak{N}}
\newcommand{\oO}{\mathfrak{O}}
\newcommand{\pP}{\mathfrak{P}}
\newcommand{\qQ}{\mathfrak{Q}}
\newcommand{\rR}{\mathfrak{R}}
\newcommand{\sS}{\mathfrak{S}}
\newcommand{\tT}{\mathfrak{T}}
\newcommand{\uU}{\mathfrak{U}}
\newcommand{\vV}{\mathfrak{V}}
\newcommand{\xX}{\mathfrak{X}}
\newcommand{\wW}{\mathfrak{W}}
\newcommand{\yY}{\mathfrak{Y}}
\newcommand{\zZ}{\mathfrak{Z}}

